Enhanced Access Traffic Steering Splitting Switching with Utility-Based Decisioning

Coexistence of 3GPP access networks, namely 4G and 5G, and non-3GPP access networks, namely Wi-Fi, has enabled data offloading from one access network to another to reduce burden on the congested network. Within the evolution of 5G system, the coexistence has been evolved to a multi-access framework where simultaneous transmission on both 3GPP and non-3GPP access networks has been enabled. This framework is named as access traffic steering, splitting and switching (ATSSS) in 3GPP and is considered as one of the key enablers to provide stringent requirements on data rate and service continuity. In this paper, we introduce an enhanced ATSSS (eAT3S) algorithm where not only instantaneous link performance measurements but also network operator preferences are taken into account to optimize the overall network performance. As part of considered non-3GPP wireless access technologies (WATs), light fidelity (LiFi) access networks are also considered alongside with Wi-Fi networks.

==> algorithmV1.tex <==
\begin{algorithm}
\caption{Enhanced ATSSS algorithm}\label{alg:eATSSS-algorithm}
%\KwData{Access network-specific telemetry data ($\tilde{x}_{\text{SINR}}$, $\tilde{x}_{\text{Buffer}}$ and $\tilde{x}_{\text{Delay}}$), measurement threshold values/parameters ($T_{\text{SINR}}$, $T_{\text{Buffer}}$ and $T_{\text{Delay}}$) and network operator preference on the considered parameter weights ($w_{\text{SINR}}$, $w_{\text{Buffer}}$ and $w_{\text{Delay}}$) are available.}
%\KwResult{Steering decision $W$: (i) selected access networks for smallest delay steering mode; or (ii) load sharing among available access networks for load balancing steering mode.}
$A \gets$ List of active users\;
\While{$A \neq \emptyset$}{
    \For{$t: $ {\upshape 5G, Wi-Fi, LiFi}}{
        \eIf{$x_{\text{SINR,t}}^u > T_{\text{SINR,t}}, ~ x_{\text{Buffer,t}}^u < T_{\text{Buffer,t}}, ~ x_{\text{Delay,t}}^u < T_{\text{Delay,t}}$}{
            {\upshape Obtain} $U_i^{t,a}$ {\upshape by} (1);
        }
        {$U_i^{t,a} = 0;$
        }
    }
    \eIf{{\upshape Steering mode: Load balancing}}{
        \For{$t: $ {\upshape 5G, Wi-Fi, LiFi}}{
        $W^{t,a} =$ $({U_i^{t,a}}/({U^{\mathrm{5G},a}+U^{\mathrm{Wi-Fi},a}+U^{\mathrm{LiFi},a}}))$x$100$;
        }
    }
    {\For{$t: $ {\upshape 5G, Wi-Fi, LiFi}}{
        \If{$U^{t,a} > 0$}{
        $W^{t,a} = 100$;
        }
    }
    }
$A \gets$ $A \setminus a$\;
}
\end{algorithm}
